Service Choreography, SBVR, and Time

We propose the use of structured natural language (English) in specifying service choreographies, focusing on the what rather than the how of the required coordination of participant services in realising a business application scenario. The declarative approach we propose uses the OMG standard Semantics of Business Vocabulary and Rules (SBVR) as a modelling language. The service choreography approach has been proposed for describing the global orderings of the invocations on interfaces of participant services. We therefore extend SBVR with a notion of time which can capture the coordination of the participant services, in terms of the observable message exchanges between them. The extension is done using existing modelling constructs in SBVR, and hence respects the standard specification. The idea is that users - domain specialists rather than implementation specialists - can verify the requested service composition by directly reading the structured English used by SBVR. At the same time, the SBVR model can be represented in formal logic so it can be parsed and executed by a machine.

==> eptcsdata.tex <==
\providecommand{\firstpage}{63}
\providecommand{\publicationstatus}{Jos\'{e} Proen\c{c}a and Massimo Tivoli (Eds.):\\
14th International Workshop on Foundations of\\
Coordination Languages and Self-Adaptive Systems (FOCLASA'15)\\
EPTCS 201, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.201.5}{10.4204/EPTCS.201.5}}
\pdfoutput=1

